Recovering 3D Hand Mesh Sequence from a Single Blurry Image: A New Dataset and Temporal Unfolding

Hands, one of the most dynamic parts of our body, suffer from blur due to their active movements. However, previous 3D hand mesh recovery methods have mainly focused on sharp hand images rather than considering blur due to the absence of datasets providing blurry hand images. We first present a novel dataset BlurHand, which contains blurry hand images with 3D groundtruths. The BlurHand is constructed by synthesizing motion blur from sequential sharp hand images, imitating realistic and natural motion blurs. In addition to the new dataset, we propose BlurHandNet, a baseline network for accurate 3D hand mesh recovery from a blurry hand image. Our BlurHandNet unfolds a blurry input image to a 3D hand mesh sequence to utilize temporal information in the blurry input image, while previous works output a static single hand mesh. We demonstrate the usefulness of BlurHand for the 3D hand mesh recovery from blurry images in our experiments. The proposed BlurHandNet produces much more robust results on blurry images while generalizing well to in-the-wild images. The training codes and BlurHand dataset are available at https://github.com/JaehaKim97/BlurHand_RELEASE.

==> latex/figures/comparison_interhand/comparison_interhand.tex <==
\begin{figure*}[t]
    \centering
    % \captionsetup[subfigure]{labelfont=scriptsize, textfont=scriptsize}
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=0.19\linewidth]{latex/figures/comparison_interhand/1807869.png} 
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-a}
        \hfill
        \includegraphics[width=0.2\linewidth]{latex/figures/comparison_interhand/1807869_mt.png}
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-a} 
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-a} 
    \end{subfigure}
    % 
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=0.19\linewidth]{latex/figures/comparison_interhand/476947.png} 
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-b}
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-b}
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-b} 
        \hfill
        \includegraphics[width=0.19\linewidth]{example-image-b}
    \end{subfigure}
    %
    \begin{subfigure}{1.0\linewidth}
        \centering
        \subfloat[Blurry image]{\includegraphics[width=0.19\linewidth]{latex/figures/comparison_interhand/722997.png}}
        \hfill
        \subfloat[Ground-truth~(center)]{\includegraphics[width=0.19\linewidth]{example-image-c}}
        \hfill
        \subfloat[METRO~\cite{lin2021end}]{\includegraphics[width=0.19\linewidth]{example-image-c}}
        \hfill
        \subfloat[Pose2Pose~\cite{moon2022accurate}]{\includegraphics[width=0.19\linewidth]{example-image-c}}
        \hfill
        \subfloat[BlurHandNet~(\textbf{Ours})]{\includegraphics[width=0.19\linewidth]{example-image-c}}
    \end{subfigure}
        
    \vspace{-1cm}
    \caption{\textbf{Qualitative results comparison with state-of-the-art methods on BlurHand.}
        %
    }
    \vspace{-0.4cm}
    \label{fig:comparison_interhand}
\end{figure*}

==> latex/sections/figures/blurhand.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur1.PNG}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur2.PNG}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur3.PNG}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur4.png}\\
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur5.png}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur6.png}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur7.png}
\includegraphics[width=0.24\linewidth]{latex/figures/blurimage/blur8png.png}
\end{center}
\caption{Examples of the proposed BlurHand dataset.}
\label{fig:example_of_dataset}
\end{figure}

==> latex/sections/figures/swin.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.98\linewidth]{latex/figures/overall/3dshift.pdf}
\end{center}
\caption{An illustration of proposed 3D shifting. While heatmaps are separated with regular size~($S_{v}$) of voxels in the first layer~(left), heatmaps are rolled in 3D dimension and divided after 3D shifting~(right).}
\label{fig:swin}
\end{figure}

==> latex/supple/figures/YT3D_comparison_last.tex <==
% \begin{figure*}[t]
%     \centering
%     \newcommand{\spacing}{3.0cm}
%     \captionsetup[subfigure]{labelfont=scriptsize, textfont=scriptsize}
%     %     \hspace*{\fill}
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/10200_B_img.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/10200_D_img.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/10200_S_mesh.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/10200_D_mesh.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/10200_B_mesh.png}}
%     %     \hspace*{\fill}
%     % \\
%     %     \hspace*{\fill}
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11166_B_img.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11166_D_img.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11166_S_mesh.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11166_D_mesh.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11166_B_mesh.png}}
%     %     \hspace*{\fill}
%     % \\
%     %     \hspace*{\fill}
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11266_B_img.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11266_D_img.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11266_S_mesh.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11266_D_mesh.png}}
%     %     \hfill
%     %     \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11266_B_mesh.png}}
%     %     \hspace*{\fill}
%     % \\
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29022_B_img.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29022_D_img.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29022_S_mesh.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29022_D_mesh.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29022_B_mesh.png}}
%     \\
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/30828_B_img.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/30828_D_img.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/30828_S_mesh.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/30828_D_mesh.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/30828_B_mesh.png}}
%     \\
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29824_B_img.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29824_D_img.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29824_S_mesh.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29824_D_mesh.png}}
%         \hfill
%         \subfloat{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/29824_B_mesh.png}}
%     \addtocounter{subfigure}{-15}
%     \\
%         \subfloat[Blurry image]{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11557_B_img.png}}
%         \hfill
%         \subfloat[Deblurred image]{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11557_D_img.png}}
%         \hfill
%         \subfloat[IH2.6M + YT3D]{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11557_S_mesh.png}}
%         \hfill
%         \subfloat[BH+\textbf{D} + YT3D]{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11557_D_mesh.png}}
%         \hfill
%         \subfloat[BH + YT3D]{\includegraphics[width=\spacing]{latex/supple/figures/YT3D/11557_B_mesh.png}}
%     % \\
% \vspace{-2mm}
%     \caption{\textbf{Effectiveness of the presented BlurHand.}
%     The captions below figures describe training sets used to train 3D hand mesh estimation networks.
%     A setting with \textbf{D} represents that the network is trained on deblurred BH and tested on (b).
%     }
%     \vspace{-0.4cm}
%     \label{fig:supple_comparison_yt3d}
% \end{figure*}

==> latex/supple/sections/1_video_format.tex <==
\section{Visualization in video format}
\label{sec_supp:video_results}
% 
% We present the video clips showing the recovered 3D meshes of our BlurHandNet with the blurry input in the supplementary videos~(\textbf{\fontfamily{pcr}\selectfont BlurHandNet.mp4}).
In the supplementary videos~(\textbf{\fontfamily{pcr}\selectfont BlurHandNet.mp4}), we visualize the recovered 3D hand mesh sequence as video clips. 
% 
In the video, we note that the left part is the input blurry hand image, and the right part is the results from our BlurHandNet.
% 
We further note that we adopt linear interpolation to smooth the motion, and motion order is determined in the order of $\mathbf{V}_{\text{E1}}$, $\mathbf{V}_{\text{M}}$, and $\mathbf{V}_{\text{E2}}$.
% 

The video shows that our BlurHandNet outputs robust 3D hand meshes from challenging blurry hand.
% 
Moreover, our BlurHandNet successfully estimates the motion in the blurry hand by performing temporal unfolding through the proposed Unfolder.
% 
Compared to the previous methods, which output the mesh in the static scene, our BlurHandNet gives more accurate and comprehensive results from blurry inputs, including motion information.
% 

==> latex/supple/sections/6_license.tex <==
\subsection*{License of the used assets}
% 

\begin{compactitem}[$\bullet$]
    \item InterHand2.6M dataset~\cite{moon2020interhand2} is CC-BY-NC 4.0 licensed.
    \item YT-3D dataset~\cite{kulon2020weakly} is Ariel AI licensed.
    \item \href{https://github.com/microsoft/MeshTransformer}{METRO~\cite{lin2021end} codes} are released for academic research only and it is free to researchers from educational or research institutes for non-commercial purposes. % code example
    \item \href{https://github.com/mks0601/Hand4Whole_RELEASE}{Pose2Pose~\cite{moon2022accurate} codes} are released for academic research only and it is free to researchers from educational or research institutes for non-commercial purposes. % code example
    \item \href{https://github.com/mks0601/I2L-MeshNet_RELEASE}{I2L-MeshNet~\cite{moon2020i2l} codes} are released for academic research only and it is free to researchers from educational or research institutes for non-commercial purposes. % code example
    
    
\end{compactitem}

\input{latex/supple/figures/YT3D_comparison_first}
\input{latex/supple/figures/BlurHand_comparison.tex}

% \input{latex/supple/figures/YT3D_comparison_last}


==> latex/supple/sections/7_comparison_under_same_cost.tex <==
\section{Number of unfolding under the same cost}
% \label
In Table~\ref{reb_tab:efficiency}, we report the performance of BlurHandNet with different numbers of unfolding steps.
Since the 
For a fair comparison, we keep the number of parameters the same by adjusting the channel size.
The results demonstrate that the performance improvement is not due to a larger network capacity.
% 
\begin{table}[!t]
    \vspace{-3mm}
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        \;~\# of unfolding & 1 & 3~(Ours) & 5\\
        \midrule
        % \,~GMACs~(\jaeha{unit}) & 13.59 & 30.02 & 46.44\\
        % \,~$\#$ of params~(M) &  & 85.36 & 85.39 \\
        \,~MPJPE (middle) & 17.48 & \textbf{16.80} & 16.91\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{\textbf{Effects of the number of unfolded hands on the BH.}}
    \label{reb_tab:efficiency}
    \vspace{-4mm}
\end{table}

==> latex/tables/5.3/dataset_effectiveness.tex <==
\begin{table}[!t]
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{C{2cm}|C{2.3cm}|C{2cm}}
\specialrule{.1em}{.05em}{.05em}
\hline
Method & Train dataset & MPJPE (mm) \\
\hline
\multirow{2}{*}{Pose2Pose} & InterHand2.6M & 25.36 \\
 & BlurHand & 18.80 \\
 \hline
\multirow{2}{*}{BlurHandNet} & Interhand2.6M & 24.57 \\
 & BlurHand & 16.80 \\
\hline
\specialrule{.1em}{.05em}{.05em}
\end{tabular}
\caption{
    \textbf{Effectiveness of BlurHand.}
}
\label{table:dataset_effectiveness}
\end{table}
